Quantum modularity and resurgence of the $q$-Pochhammer symbol

We investigate the resurgent and quantum modular properties of the logarithm of the $q$-Pochhammer symbol. From its asymptotic expansion, we compute the associated Stokes data and derive explicit formulas for its Borel--Laplace and median resummations. We show that the Borel--Laplace sums naturally encode the obstruction to modularity, leading to a quantum modular interpretation compatible with the modular resurgence paradigm of Fantini and Rella. Our results unify the two families of $q$-Pochhammer symbols studied by Fantini and Rella within a single framework, extending their results and providing further evidence for the interplay between resurgence and quantum modularity.

==> preamble.tex <==
% !TeX root = qm-qpoch.tex

\makeatletter

\usepackage{mathtools}
\mathtoolsset{showonlyrefs}
\usepackage{amssymb}
\usepackage{mathrsfs}

\usepackage{amsthm}
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

\usepackage[margin=1in]{geometry}
\usepackage{microtype}

\usepackage{iftex}
\ifpdftex
	\usepackage[T1]{fontenc}
	\usepackage{lmodern}
\else\ifluatex
	\usepackage{fontspec}
	\setmainfont{NewCM10-Book.otf}
	\setsansfont{NewCMSans10-Book.otf}
	\setmonofont{NewCMMono10-Book.otf}
	\usepackage{lua-unicode-math}
	\setmathfont{NewCMMath-Book.otf}
\fi\fi

\usepackage[dvipsnames]{xcolor}

\IfDocumentMetadataTF{}{\usepackage[inline]{enumitem}}
\setlist[enumerate,1]{
	label = (\alph*),
	font  = \upshape,
}
\setlist[enumerate,2]{
	label = (\roman*),
	font  = \upshape,
}

\usepackage[
	colorlinks        = true,
	linkcolor         = NavyBlue,
	citecolor         = NavyBlue,
	filecolor         = Red,
	urlcolor          = Red,
	menucolor         = Red,
	linktoc           = all,
	bookmarksnumbered = true,
	pdfusetitle       = true,
	pdfsubject        = {{Resurgent analysis of the q-Pochhammer symbol, including
	                      its asymptotic expansion, Borel transform, Borel–Laplace
	                      summation, median resummation, and quantum modularity.}},
	pdfkeywords       = {},
	final             = true,
]{hyperref}
\renewcommand*{\Hy@numberline}[1]{#1. }

\usepackage{bookmark}

\IfFileExists{latexml.sty}
	{\usepackage{latexml}}
	{\newif\iflatexml\latexmlfalse}
\iflatexml
	\usepackage[nameinlink]{cleveref}
	\NewDocumentCommand{\zcref}{ s o }{%
		\IfBooleanTF{#1}{\Cref*}{\Cref}%
	}
	\IfFormatAtLeastTF{2026/06/01}{}{
		\AddToHook{env/theorem/before}{\crefalias{theorem}{theorem}}
		\AddToHook{env/corollary/before}{\crefalias{theorem}{corollary}}
		\AddToHook{env/lemma/begin}{\crefalias{theorem}{lemma}}
		\AddToHook{env/proposition/begin}{\crefalias{theorem}{proposition}}
		\AddToHook{env/definition/begin}{\crefalias{theorem}{definition}}
		\AddToHook{env/remark/begin}{\crefalias{theorem}{remark}}
	}
\else
	\usepackage{zref-clever}
	\zcsetup{
		cap      = true,
		font     = \upshape,
		rangesep = {--},
		lastsep  = {, and },
	}
	\IfFormatAtLeastTF{2026/06/01}{}{
		\AddToHook{env/corollary/begin}{\zcsetup{countertype={theorem=corollary}}}
		\AddToHook{env/lemma/begin}{\zcsetup{countertype={theorem=lemma}}}
		\AddToHook{env/proposition/begin}{\zcsetup{countertype={theorem=proposition}}}
		\AddToHook{env/definition/begin}{\zcsetup{countertype={theorem=definition}}}
		\AddToHook{env/remark/begin}{\zcsetup{countertype={theorem=remark}}}
	}
	\newcommand*{\namecref}{\zcref*[nocap,noref]}
\fi

%\newcommand*{\todofont}{\scriptsize\upshape}
%\usepackage[textsize=todofont]{todonotes}
%\setlength{\marginparwidth}{2.2cm}
%\usepackage{marginnote}
%\DeclareCommandCopy{\marginpar}{\marginnote}

\usepackage{tikz}
\usetikzlibrary{math}
\usetikzlibrary{arrows.meta}


\newcommand{\km}[1]{\textcolor{magenta}{#1}} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand*{\B}{\mathcal{B}}
\newcommand*{\C}{\mathbb{C}}
\newcommand*{\e}{\mathrm{e}}
\newcommand*{\F}{\mathscr{F}}
\renewcommand*{\H}{\mathbb{H}}
\newcommand*{\M}{\mathcal{M}}
\newcommand*{\N}{\mathbb{N}}
\newcommand*{\n}{\mathbf{n}}
\newcommand*{\Q}{\mathbb{Q}}
\newcommand*{\R}{\mathbb{R}}
\renewcommand*{\S}{\mathcal{S}}
\renewcommand*{\r}{\mathbf{r}}
\newcommand*{\Z}{\mathbb{Z}}

\renewcommand*{\Re}{\operatorname{Re}}
\renewcommand*{\Im}{\operatorname{Im}}
\renewcommand*{\div}{\operatorname{div}}

\DeclareMathOperator{\disc}{disc}
\DeclareMathOperator{\SL}{SL}
\DeclareMathOperator{\Li}{Li}
\DeclareMathOperator{\Res}{Res}
\DeclareMathOperator{\Den}{Den}
\DeclareMathOperator{\PV}{PV}

\newcommand*{\slog}{\log^*}
\newcommand*{\ol}[1]{\overline{#1}}
\newcommand*{\sm}{\setminus}
\newcommand*{\pd}{\partial}
\newcommand*{\psum}{\sideset{}{'}{\sum}}
\newcommand*{\Smed}{\mathcal{S}^{\mathrm{med}}}
\newcommand*{\tf}{\tilde{f}}
\newcommand*{\tF}{\widetilde{F}}
\newcommand*{\tFF}{\widetilde{\F}}
\newcommand*{\tr}{\tilde{\r}}

\renewcommand*{\le}{\leqslant}
\renewcommand*{\ge}{\geqslant}
\renewcommand*{\leq}{\leqslant}
\renewcommand*{\geq}{\geqslant}
\renewcommand*{\qedsymbol}{$\blacksquare$}

\newcommand*{\qand}{\quad \text{and} \quad}
\newcommand*{\qqand}{\qquad \text{and} \qquad}
\newcommand*{\qor}{\quad \text{or} \quad}
\newcommand*{\qqor}{\qquad \text{or} \qquad}

\DeclarePairedDelimiterX{\@qpoch}[2]{(}{)}{#1;#2}
\NewDocumentCommand{\qpoch}{ s O{} m m O{\infty} }{%
	\IfBooleanTF{#1}{\def\@temp{*}}{\def\@temp{[#2]}}%
	\expandafter\@qpoch\@temp{#3}{#4}_{#5}%
}

\NewCommandCopy{\@originalmod}{\mod}
\RenewDocumentCommand{\mod}{ s m }{%
	\IfBooleanTF{#1}
		{\mkern8mu{\operator@font mod}\mkern6mu#2}
		{\@originalmod{#2}}
}

\NewCommandCopy{\@originalpmod}{\pmod}
\RenewDocumentCommand{\pmod}{ s m }{%
	\IfBooleanTF{#1}
		{\mkern6mu({\operator@font mod}\mkern6mu#2)}
		{\@originalpmod{#2}}
}

\NewCommandCopy{\@originalsqrt}{\sqrt}
\RenewDocumentCommand{\sqrt}{ o }{%
	\IfNoValueTF{#1}{\@originalsqrt}{\mspace{-1mu}\@originalsqrt[#1]}%
}

\NewCommandCopy{\@originalleft}{\left}
\NewCommandCopy{\@originalright}{\right}
\renewcommand*{\left}{\mathopen{}\mathclose\bgroup\@originalleft}
\renewcommand*{\right}{\aftergroup\egroup\@originalright}

\DeclarePairedDelimiter{\@abs}{\lvert}{\rvert}
\newcommand*{\abs}{{}\@abs}

\DeclarePairedDelimiter{\@floor}{\lfloor}{\rfloor}
\newcommand*{\floor}{{}\@floor}

\DeclarePairedDelimiter{\@ceil}{\lceil}{\rceil}
\newcommand*{\ceil}{{}\@ceil}

\NewDocumentCommand{\prmatrix}{ s m m o o o }{%
	\IfBooleanTF{#1}%
		{\begin{psmallmatrix} #2 \\ #3 \IfValueT{#4}{\\ #4} \IfValueT{#5}{\\ #5} \IfValueT{#6}{\\ #6} \end{psmallmatrix}}%
		{\begin{pmatrix}      #2 \\ #3 \IfValueT{#4}{\\ #4} \IfValueT{#5}{\\ #5} \IfValueT{#6}{\\ #6} \end{pmatrix}     }%
}


\IfClassLoadedTF{amsart}{}{
	\providecommand*{\NoHyper}{}
	\newcommand{\@footnote}[1]{%
		\begin{NoHyper}
			\def\@thefnmark{}%
			\@footnotetext{#1}%
		\end{NoHyper}%
	}
	\newcommand*{\subjclass}[2][2020]{%
		\AddToHook{cmd/maketitle/after}{\@footnote{#1 \textit{Mathematics Subject Classification}. #2}}%
	}
	\newcommand*{\keywords}[1]{%
		\AddToHook{cmd/maketitle/after}{\@footnote{\textit{Key words and phrases}. #1}}%
		\IfPackageLoadedTF{hyperref}{\hypersetup{pdfkeywords = {#1}}}{}%
	}
}

\AddToHook{cmd/bibliography/before}{%
	\IfDocumentMetadataTF
		{\AddToHookNext{cmd/section/after}{\addcontentsline{toc}{section}{\refname}}}
		{\AddToHookNext{cmd/@xsect/after} {\addcontentsline{toc}{section}{\refname}}}
}

\NewDocumentCommand{\scalewidth}{ O{0.5} O{c} m }{%
	\ifmmode
	\mathchoice
		{\@scalewidth{#1}{#2}{$\m@th\displaystyle#3$}}
		{\@scalewidth{#1}{#2}{$\m@th\textstyle#3$}}
		{\@scalewidth{#1}{#2}{$\m@th\scriptstyle#3$}}
		{\@scalewidth{#1}{#2}{$\m@th\scriptscriptstyle#3$}}%
	\else
		\@scalewidth{#1}{#2}{#3}%
	\fi
}

\newcommand*{\@scalewidth}[3]{%
	\settowidth{\@tempskipa}{#3}%
	\makebox[\dimexpr #1\@tempskipa][#2]{#3}%
}

\allowdisplaybreaks[4]

\DeclareFontFamily{U}{rcjhbltx}{}
\DeclareFontShape{U}{rcjhbltx}{m}{n}{<->rcjhbltx}{}
\DeclareSymbolFont{hebrewletters}{U}{rcjhbltx}{m}{n}
\DeclareMathSymbol{\shin}{\mathord}{hebrewletters}{152}

\counterwithin{equation}{section}
\counterwithin{figure}{section}

\makeatother
